Completeness of Datasets Documentation on ML/AI repositories: an Empirical Investigation

ML/AI is the field of computer science and computer engineering that arguably received the most attention and funding over the last decade. Data is the key element of ML/AI, so it is becoming increasingly important to ensure that users are fully aware of the quality of the datasets that they use, and of the process generating them, so that possible negative impacts on downstream effects can be tracked, analysed, and, where possible, mitigated. One of the tools that can be useful in this perspective is dataset documentation. The aim of this work is to investigate the state of dataset documentation practices, measuring the completeness of the documentation of several popular datasets in ML/AI repositories. We created a dataset documentation schema -- the Documentation Test Sheet (DTS) -- that identifies the information that should always be attached to a dataset (to ensure proper dataset choice and informed use), according to relevant studies in the literature. We verified 100 popular datasets from four different repositories with the DTS to investigate which information was present. Overall, we observed a lack of relevant documentation, especially about the context of data collection and data processing, highlighting a paucity of transparency.

==> tables/doc-test-sheet.tex <==
\begin{longtable}[c]{|p{0.1\textwidth}|p{0.725\textwidth}|p{0.1\textwidth}|}
    \caption{Documentation Test Sheet} \label{tab:documentation-test-sheet} \\

    \hline \multicolumn{3}{|l|}{\footnotesize\textbf{Dataset:}} \\ \hline \multicolumn{1}{|p{0.1\textwidth}|}{\footnotesize\textbf{Test Field ID}} & \multicolumn{1}{p{0.725\textwidth}|}{\footnotesize\textbf{Test Field Name}} & \multicolumn{1}{p{0.1\textwidth}|}{\footnotesize\textbf{Presence Check}} \\ \hline
    \endfirsthead

    \multicolumn{3}{c}%
    {\tablename\ \thetable{} -- continued from previous page} \\
    \hline \multicolumn{3}{|l|}{\footnotesize\textbf{Dataset:}} \\ \hline \multicolumn{1}{|p{0.1\textwidth}|}{\footnotesize\textbf{Test Field ID}} & \multicolumn{1}{p{0.725\textwidth}|}{\footnotesize\textbf{Test Field Name}} & \multicolumn{1}{p{0.1\textwidth}|}{\footnotesize\textbf{Presence Check}} \\ \hline
    \endhead

    \hline \multicolumn{3}{|r|}{{Continue on next page}} \\ \hline
    \endfoot

    \hline
    \endlastfoot

    \hline
    1.01 & \textit{Purpose for the dataset creation} &  \\ \hline
    1.02 & \textit{Dataset creators} &  \\ \hline
    1.03 & \textit{Dataset funders} &  \\ \hline
    \multicolumn{2}{|r|}{\textbf{1} \textit{Motivation} \textit{Presence Average}} & \\ \hline 
    2.01 & \textit{Description of the instances} &  \\ \hline
    2.02 & \textit{Number of the instances} &  \\ \hline
    2.03 & \textit{Information about missing values} &  \\ \hline
    2.04 & \textit{Recommended data splits} &  \\ \hline
    2.05 & \textit{Description of errors, noise or redundancies} &  \\ \hline
    2.06 & \textit{Information about data confidentiality} &  \\ \hline
    2.07 & \textit{Information about possible data dangerousness (offensive, insulting, threatening or cause anxiety) or biases} &  \\ \hline
    2.08 & \textit{Information about people involved in data production and their compensation (if people related)} &  \\ \hline
    2.09 & \textit{Description of identifiability for individuals or subpopulations (if people related)} &  \\ \hline
    2.10 & \textit{Description of  data sensitivity (if people related)} &  \\ \hline
    2.11 & \textit{Statistics} &  \\ \hline
    2.12 & \textit{Pair plots} &  \\ \hline
    2.13 & \textit{Probabilistic model} &  \\ \hline
    2.14 & \textit{Ground truth correlations} &  \\ \hline
    \multicolumn{2}{|r|}{\textbf{2} \textit{Composition} \textit{Presence Average}} & \\ \hline
    3.01 & \textit{Description of instances acquisition and data collection processes} &  \\ \hline
    3.02 & \textit{Information about people involved in the data collection process and their compensation} &  \\ \hline
    3.03 & \textit{Time frame of data collection} &  \\ \hline
    3.04 & \textit{Information about ethical review processes} &  \\ \hline
    3.05 & \textit{Information on individuals' knowledge of data collection (if people related)} &  \\ \hline
    3.06 & \textit{Information on individuals' consent for data collection (if people related)} &  \\ \hline
    3.07 & \textit{Analysis of potential impacts of the dataset and its use on data subjects} &  \\ \hline
    \multicolumn{2}{|r|}{\textbf{3} \textit{Collection processes} \textit{Presence Average}} & \\ \hline \pagebreak
    4.01 & \textit{Description of sampling, preprocessing, cleaning, labelling procedures} &  \\ \hline
    4.02 & \textit{Information about people involved in the data sampling, preprocessing, cleaning, labelling procedures and their compensation} &  \\ \hline
    4.03 & \textit{Description of others possible sampling, preprocessing, cleaning, labelling procedures} &  \\ \hline
    \multicolumn{2}{|r|}{\textbf{4} \textit{Data processing procedures} \textit{Presence Average}} & \\ \hline
    5.01 & \textit{Description of the tasks in which the dataset has already been used and their results} &  \\ \hline
    5.02 & \textit{Description of recommended uses or tasks} &  \\ \hline
    5.03 & \textit{Description of not recommended uses} &  \\ \hline
    5.04 & \textit{Repository that links to papers or system that use the datasets} &  \\ \hline
    5.05 & \textit{Description of license and terms of use} &  \\ \hline
    \multicolumn{2}{|r|}{\textbf{5} \textit{Uses} \textit{Presence Average}} & \\ \hline
    6.01 & \textit{Information about subject supporting, hosting, maintaining the dataset} &  \\ \hline
    6.02 & \textit{Contact of the owner} &  \\ \hline
    6.03 & \textit{DOI} &  \\ \hline
    6.04 & \textit{Erratum} &  \\ \hline
    6.05 & \textit{Information about dataset updates} &  \\ \hline
    6.06 & \textit{Information about management of older dataset versions} &  \\ \hline
    6.07 & \textit{Information about the mechanism to extend, augment, build on, contribute to the dataset} &  \\ \hline
    \multicolumn{2}{|r|}{\textbf{6} \textit{Maintenance} \textit{Presence Average}} & \\ \hline

    \multicolumn{2}{|r|}{Dataset \textit{Presence Average}} & \\ \hline
    
    \multicolumn{2}{|l|}{Dataset \textit{Characteristics}} & \\ \hline
    c.01 & \textit{Data is people related} &  \\ \hline
    c.02 & \textit{Presence of explicit target variable} &  \\ \hline
    c.03 & \textit{Dataset is a sample or a reduction of a larger set} &  \\ \hline
    c.04 & \textit{Recently updated} &  \\ \hline
\end{longtable}

==> tables/selected-datasets.tex <==
\begin{table}[h]
    \caption{Huggingface selected datasets (20/11/2021)}
    \label{tab:datasets-huggingface}
    % \centering 
    \raggedright
    % \begin{tabular}{|l|l|c|l|m{4cm}|}
    \begin{tabular}{|m{1cm}|m{3.6cm}|m{1cm}|m{1cm}|m{5.5cm}|}
    \hline \multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Download}} & \multicolumn{1}{c|}{\textbf{Duplicate of}} & \multicolumn{1}{c|}{\textbf{URL}} \\ \hline

    hug01 & glue             & 719706 &  & \url{https://huggingface.co/datasets/glue}             \\
    hug02 & super\_glue      & 490789 &  & \url{https://huggingface.co/datasets/super_glue}      \\
    hug03 & anli             & 171100 &  & \url{https://huggingface.co/datasets/anli}             \\
    hug04 & wikitext         & 114761 &  & \url{https://huggingface.co/datasets/wikitext}         \\
    hug05 & wino\_bias       & 102485 &  & \url{https://huggingface.co/datasets/wino_bias}       \\
    hug06 & squad            & 98446  &  & \url{https://huggingface.co/datasets/squad}            \\
    hug07 & imdb             & 93646  &  & \url{https://huggingface.co/datasets/imdb}             \\
    hug08 & trec             & 71906  &  & \url{https://huggingface.co/datasets/trec}             \\
    hug09 & adversarial\_qa  & 70084  &  & \url{https://huggingface.co/datasets/adversarial_qa}  \\
    hug10 & race             & 68456  &  & \url{https://huggingface.co/datasets/race}             \\
    hug11 & duorc            & 67179  &  & \url{https://huggingface.co/datasets/duorc}            \\
    hug12 & squad\_v2        & 66750  &  & \url{https://huggingface.co/datasets/squad_v2}        \\
    hug13 & winogrande       & 58213  &  & \url{https://huggingface.co/datasets/winogrande}       \\
    hug14 & hellaswag        & 54372  &  & \url{https://huggingface.co/datasets/hellaswag}        \\
    hug15 & common\_voice    & 54179  &  & \url{https://huggingface.co/datasets/common_voice}    \\
    hug16 & cnn\_dailymail   & 53207  &  & \url{https://huggingface.co/datasets/cnn_dailymail}   \\
    hug17 & piqa             & 53155  &  & \url{https://huggingface.co/datasets/piqa}             \\
    hug18 & xsum             & 50393  &  & \url{https://huggingface.co/datasets/xsum}             \\
    hug19 & cosmos\_qa       & 50151  &  & \url{https://huggingface.co/datasets/cosmos_qa}       \\
    hug20 & mlqa             & 49740  &  & \url{https://huggingface.co/datasets/mlqa}             \\
    hug21 & quail            & 49413  &  & \url{https://huggingface.co/datasets/quail}            \\
    hug22 & paws             & 48998  &  & \url{https://huggingface.co/datasets/paws}             \\
    hug23 & wmt16            & 48694  &  & \url{https://huggingface.co/datasets/wmt16}            \\
    hug24 & ai2\_arc         & 47424  &  & \url{https://huggingface.co/datasets/ai2_arc}         \\
    hug25 & rotten\_tomatoes & 46131  &  & \url{https://huggingface.co/datasets/rotten_tomatoes} \\
%    hug26 & ropes            & 45861  &  & \url{https://huggingface.co/datasets/ropes}            \\
%    hug27 & ag\_news         & 45359  &  & \url{https://huggingface.co/datasets/ag_news}         \\
%    hug28 & amazon\_polarity & 44621  &  & \url{https://huggingface.co/datasets/amazon_polarity} \\
%    hug29 & cos\_e           & 43434  &  & \url{https://huggingface.co/datasets/cos_e}           \\
%    hug30 & wiki\_qa         & 42721  &  & \url{https://huggingface.co/datasets/wiki_qa}         \\
    \hline 
\end{tabular}\end{table}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{longtable}[c]{|m{1cm}|m{3.6cm}|m{1cm}|m{1cm}|m{5.5cm}|}
    \caption{Kaggle selected datasets (18/11/2021)} \label{tab:datasets-kaggle} \\
    
    \hline \multicolumn{1}{|c|}{\footnotesize\textbf{ID}} & \multicolumn{1}{c|}{\footnotesize\textbf{Name}} & \multicolumn{1}{c|}{\footnotesize\textbf{Download}} & \multicolumn{1}{c|}{\footnotesize\textbf{Duplicate of}} & \multicolumn{1}{c|}{\footnotesize\textbf{URL}} \\ \hline
    \endfirsthead

    \multicolumn{5}{c}%
    {{\tablename\ \thetable{} -- continued from previous page}} \\
    \hline \multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Download}} & \multicolumn{1}{c|}{\textbf{Duplicate of}} & \multicolumn{1}{c|}{\textbf{URL}} \\ \hline
    \endhead

    \hline \multicolumn{5}{|r|}{{Continue on next page}} \\ \hline
    \endfoot

    \hline
    \endlastfoot
    
    kag01 & Credit Card Fraud Detection                         & 360828 &       & \url{https://www.kaggle.com/mlg-ulb/creditcardfraud}                            \\
    kag02 & Novel Corona Virus 2019 Dataset                     & 347779 &       & \url{https://www.kaggle.com/sudalairajkumar/novel-corona-virus-2019-dataset}    \\
    kag03 & Video Game Sales                                    & 264773 &       & \url{https://www.kaggle.com/gregorut/videogamesales}                            \\
    kag04 & Heart Disease UCI                                   & 256102 & uci04 & \url{https://www.kaggle.com/ronitf/heart-disease-uci}                           \\
    kag05 & Pima Indians Diabetes Database                      & 235317 & oml04 & \url{https://www.kaggle.com/uciml/pima-indians-diabetes-database}               \\
    kag06 & Iris Species                                        & 228045 & uci01 & \url{https://www.kaggle.com/uciml/iris}                                         \\
    kag07 & World Happiness Report                              & 202882 &       & \url{https://www.kaggle.com/unsdsn/world-happiness}                             \\
    kag08 & Netflix Movies and TV Shows                         & 183020 &       & \url{https://www.kaggle.com/shivamb/netflix-shows}                              \\
    kag09 & The Movies Dataset                                  & 178101 &       & \url{https://www.kaggle.com/rounakbanik/the-movies-dataset}                     \\
    kag10 & Breast Cancer Wisconsin (Diagnostic) Data Set       & 177162 & uci07 & \url{https://www.kaggle.com/uciml/breast-cancer-wisconsin-data}                 \\
    kag11 & TMDB 5000 Movie Dataset                             & 174636 &       & \url{https://www.kaggle.com/tmdb/tmdb-movie-metadata}                           \\
    kag12 & COVID-19 Dataset                                    & 168132 & kag02 & \url{https://www.kaggle.com/imdevskp/corona-virus-report}                       \\
    kag13 & Google Play Store Apps                              & 166169 &       & \url{https://www.kaggle.com/lava18/google-play-store-apps}                      \\
    kag14 & Trending YouTube Video Statistics                   & 158082 &       & \url{https://www.kaggle.com/datasnaek/youtube-new}                              \\
    kag15 & Wine Reviews                                        & 148561 &       & \url{https://www.kaggle.com/zynicide/wine-reviews}                              \\
    kag16 & Chest X-Ray Images (Pneumonia)                      & 143227 &       & \url{https://www.kaggle.com/paultimothymooney/chest-xray-pneumonia}             \\
    kag17 & European Soccer Database                            & 140647 &       & \url{https://www.kaggle.com/hugomathien/soccer}                                 \\
    kag18 & COVID-19 in India                                   & 137213 &       & \url{https://www.kaggle.com/sudalairajkumar/covid19-in-india}                   \\
    kag19 & COVID-19 Open Research Dataset Challenge (CORD-19)  & 134256 &       & \url{https://www.kaggle.com/allen-institute-for-ai/CORD-19-research-challenge}  \\
    kag20 & Students Performance in Exams                       & 134210 &       & \url{https://www.kaggle.com/spscientist/students-performance-in-exams}          \\
    kag21 & FIFA 19 complete player dataset                     & 130521 &       & \url{https://www.kaggle.com/karangadiya/fifa19}                                 \\
    kag22 & Avocado Prices                                      & 126093 &       & \url{https://www.kaggle.com/neuromusic/avocado-prices}                          \\
    kag23 & House Sales in King County, USA                     & 111243 &       & \url{https://www.kaggle.com/harlfoxem/housesalesprediction}                     \\
    kag24 & Suicide Rates Overview 1985 to 2016                 & 111006 &       & \url{https://www.kaggle.com/russellyates88/suicide-rates-overview-1985-to-2016} \\
    kag25 & New York City Airbnb Open Data                      & 110090 &       & \url{https://www.kaggle.com/dgomonov/new-york-city-airbnb-open-data}            \\
    kag26 & Red Wine Quality                                    & 108089 &       & \url{https://www.kaggle.com/uciml/red-wine-quality-cortez-et-al-2009}           \\
    kag27 & Amazon Fine Food Reviews                            & 108069 &       & \url{https://www.kaggle.com/snap/amazon-fine-food-reviews}                      \\
    kag28 & Fashion MNIST                                       & 102001 &       & \url{https://www.kaggle.com/zalando-research/fashionmnist}                      \\
    kag29 & Telco Customer Churn                                & 101166 &       & \url{https://www.kaggle.com/blastchar/telco-customer-churn}                     \\
    kag30 & Bitcoin Historical Data                             & 98823  &       & \url{https://www.kaggle.com/mczielinski/bitcoin-historical-data}                \\
%    kag31 & Brazilian E-Commerce Public Dataset by Olist        & 96837  &       & \url{https://www.kaggle.com/olistbr/brazilian-ecommerce}                        \\
%    kag32 & Medical Cost Personal Datasets                      & 94918  &       & \url{https://www.kaggle.com/mirichoi0218/insurance}                             \\
%    kag33 & {[}NeurIPS 2020{]} Data Science for COVID-19 (DS4C) & 93132  &       & \url{https://www.kaggle.com/kimjihoo/coronavirusdataset}                        \\
%    kag34 & Student Alcohol Consumption                         & 88475  &       & \url{https://www.kaggle.com/uciml/student-alcohol-consumption}                  \\
%    kag35 & IBM HR Analytics Employee Attrition \& Performance  & 85307  &       & \url{https://www.kaggle.com/pavansubhasht/ibm-hr-analytics-attrition-dataset}   \\
    % \hline
\end{longtable}
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{longtable}[c]{|m{1cm}|m{3.6cm}|m{1cm}|m{1cm}|m{5.5cm}|}
    \caption{UC Irvine Machine Learning Repository selected datasets (27/01/2022)} \label{tab:datasets-ucimlr} \\
    
    \hline \multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Download}} & \multicolumn{1}{c|}{\textbf{Duplicate of}} & \multicolumn{1}{c|}{\textbf{URL}} \\ \hline
    \endfirsthead

    \multicolumn{5}{c}%
    {{\tablename\ \thetable{} -- continued from previous page}} \\

    \hline \multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Download}} & \multicolumn{1}{c|}{\textbf{Duplicate of}} & \multicolumn{1}{c|}{\textbf{URL}} \\ \hline
    \endhead
    
    \hline \multicolumn{5}{|r|}{{Continue on next page}} \\ \hline
    \endfoot

    \hline
    \endlastfoot
    
    uci01 & Iris                                         & 122721 &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/iris}                                         \\
    uci02 & Diabetes                                     & 85583  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/diabetes}                                     \\
    uci03 & Adult                                        & 81206  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/adult}                                        \\
    uci04 & Heart Disease                                & 77318  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/heart+disease}                                \\
    uci05 & Wine                                         & 63145  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/wine}                                         \\
    uci06 & Car Evaluation                               & 60395  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/car+evaluation}                               \\
    uci07 & Breast Cancer Wisconsin (Diagnostic)         & 54593  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/breast+cancer+wisconsin+diagnostic}           \\
    uci08 & Abalone                                      & 45356  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/abalone}                                      \\
    uci09 & Breast Cancer                                & 44779  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/breast+cancer}                                \\
    uci10 & Mushroom                                     & 44738  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/mushroom}                                     \\
    uci11 & Glass Identification                         & 40148  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/glass+identification}                         \\
    uci12 & Census Income                                & 34569  & uci03 & \url{https://archive-beta.ics.uci.edu/ml/datasets/census+income}                                \\
    uci13 & Breast Cancer Wisconsin (Original)           & 33993  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/breast+cancer+wisconsin+original}             \\
    uci14 & Statlog (German Credit Data)                 & 33688  & oml01 & \url{https://archive-beta.ics.uci.edu/ml/datasets/statlog+german+credit+data}                   \\
    uci15 & Thyroid Disease                              & 28521  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/thyroid+disease}                              \\
    uci16 & Liver Disorders                              & 28141  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/liver+disorders}                              \\
    uci17 & Optical Recognition of Handwritten Digits    & 27391  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/optical+recognition+of+handwritten+digits}    \\
    uci18 & Ionosphere                                   & 26767  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/ionosphere}                                   \\
    uci19 & Auto MPG                                     & 26543  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/auto+mpg}                                     \\
    uci20 & Pen-Based Recognition of Handwritten Digits  & 26233  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/pen+based+recognition+of+handwritten+digits}  \\
    uci21 & Image Segmentation                           & 24985  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/image+segmentation}                           \\
    uci22 & Congressional Voting Records                 & 24684  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/congressional+voting+records}                 \\
    uci23 & Zoo                                          & 24438  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/zoo}                                          \\
    uci24 & Letter Recognition                           & 23194  & oml10 & \url{https://archive-beta.ics.uci.edu/ml/datasets/letter+recognition}                           \\
    uci25 & Lung Cancer                                  & 23075  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/lung+cancer}                                  \\
    uci26 & Spambase                                     & 21980  & oml08 & \url{https://archive-beta.ics.uci.edu/ml/datasets/spambase}                                     \\
    uci27 & Yeast                                        & 21867  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/yeast}                                        \\
    uci28 & Hepatitis                                    & 21415  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/hepatitis}                                    \\
    uci29 & Internet Advertisements                      & 20802  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/internet+advertisements}                      \\
%    uci30 & Statlog Project                              & 19909  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/statlog+project}                              \\
%    uci31 & Reuters-21578 Text Categorization Collection & 19490  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/reuters+21578+text+categorization+collection} \\
%    uci32 & Connectionist Bench (Sonar, Mines vs. Rocks) & 19180  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/connectionist+bench+sonar+mines+vs+rocks}     \\
%    uci33 & Tic-Tac-Toe Endgame                          & 19051  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/tic+tac+toe+endgame}                          \\
%    uci34 & Soybean (Large)                              & 18865  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/soybean+large}                                \\
%    uci35 & Soybean (Small)                              & 18739  &       & \url{https://archive-beta.ics.uci.edu/ml/datasets/soybean+small}                                \\
    \hline

\end{longtable}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h]
    \centering
    \caption{OpenML selected datasets (03/02/2022)}
    \label{tab:datasets-openml}
    \begin{tabular}{|m{1cm}|m{3.6cm}|m{1cm}|m{1cm}|m{5.5cm}|}
    \hline \multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Download}} & \multicolumn{1}{c|}{\textbf{Duplicate of}} & \multicolumn{1}{c|}{\textbf{URL}} \\ \hline
    oml01 & credit-g (1)                         & 302 &       & \url{https://www.openml.org/d/31}    \\
    oml02 & SpeedDating (1)                      & 168 &       & \url{https://www.openml.org/d/40536} \\
    oml03 & iris (1)                             & 157 & uci01 & \url{https://www.openml.org/d/61}    \\
    oml04 & diabetes (1)                         & 104 &       & \url{https://www.openml.org/d/37}    \\
    oml05 & blood-transfusion-service-center (1) & 100 &       & \url{https://www.openml.org/d/1464}  \\
    oml06 & tic-tac-toe (1)                      & 96  &       & \url{https://www.openml.org/d/50}    \\
    oml07 & eeg-eye-state (1)                    & 95  &       & \url{https://www.openml.org/d/1471}  \\
    oml08 & spambase (1)                         & 93  &       & \url{https://www.openml.org/d/44}    \\
    oml09 & mnist\_784 (1)                       & 81  &       & \url{https://www.openml.org/d/554}   \\
    oml10 & letter (1)                           & 75  &       & \url{https://www.openml.org/d/6}     \\
    oml11 & isolet (1)                           & 71  &       & \url{https://www.openml.org/d/300}   \\
    oml12 & Satellite (1)                        & 70  &       & \url{https://www.openml.org/d/40900} \\
    oml13 & one-hundred-plants-texture (1)       & 67  &       & \url{https://www.openml.org/d/1493}  \\
    oml14 & creditcard (1)                       & 59  & kag01 & \url{https://www.openml.org/d/1597}  \\
    oml15 & soybean (1)                          & 56  &       & \url{https://www.openml.org/d/42}    \\
    oml16 & waveform-5000 (1)                    & 54  &       & \url{https://www.openml.org/d/60}    \\
    oml17 & gisette (2)                          & 53  &       & \url{https://www.openml.org/d/41026} \\
    oml18 & glass (1)                            & 52  & uci11 & \url{https://www.openml.org/d/41}    \\
    oml19 & steel-plates-fault (1)               & 50  &       & \url{https://www.openml.org/d/1504}  \\
    oml20 & arrhythmia (1)                       & 50  &       & \url{https://www.openml.org/d/5}     \\
    oml21 & mammography (1)                      & 49  &       & \url{https://www.openml.org/d/310}   \\
    oml22 & amazon-commerce-reviews (1)          & 48  &       & \url{https://www.openml.org/d/1457}  \\
    oml23 & electricity (1)                      & 45  &       & \url{https://www.openml.org/d/151}   \\
    oml24 & kr-vs-kp (1)                         & 44  &       & \url{https://www.openml.org/d/3}     \\
    oml25 & spectrometer (1)                     & 44  &       & \url{https://www.openml.org/d/313}   \\
    oml26 & mushroom (1)                         & 42  & uci10 & \url{https://www.openml.org/d/24}    \\
    oml27 & Titanic (1)                          & 42  &       & \url{https://www.openml.org/d/40945} \\
    oml28 & bank-marketing (1)                   & 41  &       & \url{https://www.openml.org/d/1461}  \\
    oml29 & phoneme (1)                          & 40  &       & \url{https://www.openml.org/d/1489}  \\
%    oml30 & one-hundred-plants-shape (1)         & 40  &       & \url{https://www.openml.org/d/1492}  \\
%    oml31 & Bioresponse (1)                      & 40  &       & \url{https://www.openml.org/d/4134}  \\
%    oml32 & covertype (3)                        & 40  &       & \url{https://www.openml.org/d/150}   \\
%    oml33 & wdbc (1)                             & 39  &       & \url{https://www.openml.org/d/1510}  \\
%    oml34 & banknote-authentication (1)          & 39  &       & \url{https://www.openml.org/d/1462}  \\
%    oml35 & breast-cancer (1)                    & 37  &       & \url{https://www.openml.org/d/13}    \\
    \hline
    \end{tabular}
\end{table}
